Growing an Agent/Prover Interface: Evolutionary Tool Design for Cost-Efficient Theorem Proving in Rocq and Lean

Recent achievements in AI-assisted mathematics require intensive interaction of agents with proof assistants to generate machine-checked proof certificates. Agents interact with proof assistants such as Rocq or Lean through an interface that controls what the agent receives from the prover and the cost of these interactions. Today, these interfaces are adapted from tools designed for humans and not optimized for agents. We propose an evolutionary method where a frontier model incrementally proposes new features and only keeps the ones that improve the overall performance of smaller models. We demonstrate the effectiveness of our method by growing, on a curated set of mathematical problems, ROCQ-MCP-EVOLVE, a new MCP server for the Rocq prover. On the held-out test split of miniF2F-Rocq, an agent equipped with ROCQ-MCP-EVOLVE outperforms both the baseline that only exposes the Rocq compiler and an established MCP server, across four models from two families, in success rate, cost per solve, and time per solve. Although evolved for Rocq, the resulting server transfers to Lean, improving cost and time per solve on a subset of PutnamBench. We release ROCQ-MCP-EVOLVE and its port to Lean.

==> figures/barchart-defs.tex <==
% Reusable TikZ definitions for bar-chart figures.
%
% Usage: from any .tex file in this figures/ folder, load once with
%   \input{figures/barchart-defs.tex}
% before the tikzpicture that uses these commands. Requires \usepackage{tikz}
% (already loaded by iclr2027_conference.tex).

\usetikzlibrary{calc}
\usetikzlibrary{patterns.meta}

% The list-helper macros below (\nthitem, \splitpair) grab an item out of a
% list via \xdef/\edef. A plain \edef fully executes whatever it finds,
% which breaks if a list item is (or expands to) a robust/font-switching
% command such as \textsc (used e.g. by \rme's \textsc{...}\xspace
% definition in macros.tex): \edef would run its internals instead of
% leaving it inert, corrupting the result. \protected@edef/\protected@xdef
% are the standard LaTeX-kernel replacements that pass such commands
% through unexecuted, so aliases built on \textsc survive being put in a
% list like \toolings. Needs \makeatletter since they contain "@".
\makeatletter

% Layout: bars are horizontal. A diagram's origin (0,0) is the top-left
% corner of its plot area; categories (bars/groups) run downward from it,
% and values grow rightwards from the baseline x=0 over \barchartlength
% (cm) for the [vmin,vmax] range. The "span" arguments below are the
% diagram's extent along the category direction (downward), in cm.

% Geometry parameters, in cm/data units. Redefine to override.
\providecommand{\barchartlength}{4}

\tikzset{
  bar axis/.style={draw, black, thick},
  bar grid/.style={draw, gray!30, thin},
  bar label/.style={font=\small, black},
  bar value label/.style={font=\scriptsize, black, anchor=west},
  bar tick label/.style={font=\scriptsize, black},
}

% Geometry of the striped/dotted fill patterns. Redefine before \input to
% override (uses patterns.meta, so these keys -- distance, radius, line
% width -- are real, unlike the fixed-spacing plain "patterns" library).
\providecommand{\dotpatterndistance}{1.5pt}
\providecommand{\dotpatternradius}{0.4pt}
\providecommand{\stripepatterndistance}{2pt}
\providecommand{\stripepatternlinewidth}{0.4pt}
\providecommand{\stripepatternangle}{45}

% Bar-filling settings, selectable by name ("full", "striped", "dotted")
% from \drawbar's pattern argument. Each takes the bar's color as an
% argument, e.g. used as [bar fill striped={haikucolor}].
\tikzset{
  bar fill full/.style={fill=#1},
  bar fill striped/.style={
    pattern={Lines[angle=\stripepatternangle, distance=\stripepatterndistance, line width=\stripepatternlinewidth]},
    pattern color=#1},
  bar fill dotted/.style={
    pattern={Dots[distance=\dotpatterndistance, radius=\dotpatternradius]},
    pattern color=#1},
}

% \baraxes{span}: draw the category baseline (vertical, at x=0) and the
% value axis (horizontal, along the bottom of the diagram).
\newcommand{\baraxes}[1]{%
  \draw[bar axis] (0,0) -- (0,-#1);
  \draw[bar axis] (0,-#1) -- (\barchartlength,-#1);
}

% \bargridlines{span}{vmin}{vmax}{vstep}: vertical gridlines with value tick
% labels below the value axis, from vmin to vmax every vstep data units.
% vstep should evenly divide (vmax-vmin); \bargridlinesN{span}{vmin}{vmax}{n}
% below picks vstep automatically for n equal gridline gaps.
\newcommand{\bargridlines}[4]{%
  % floor(...+epsilon): see \vaxisgridlines for why -- (vmax-vmin)/vstep
  % should be an exact integer, but floating point can land it a hair
  % under, silently dropping the last gridline from the {0,...,n} loop.
  \pgfmathsetmacro{\nsteps}{floor((#3-#2)/#4+0.001)}
  \foreach \i in {0,...,\nsteps} {
    \pgfmathsetmacro{\tickval}{#2+\i*#4}
    \pgfmathsetmacro{\tickpos}{(\tickval-#2)/(#3-#2)*\barchartlength}
    \draw[bar grid] (\tickpos,0) -- (\tickpos,-#1);
    \node[bar tick label, anchor=north] at (\tickpos,-#1-0.1) {\pgfmathprintnumber[fixed,precision=3,zerofill=false]{\tickval}};
  }
}

% \bargridlinesN{span}{vmin}{vmax}{n}: like \bargridlines, but takes a
% number of equal gridline gaps `n` instead of an explicit step.
\newcommand{\bargridlinesN}[4]{%
  \pgfmathsetmacro{\bargridlinesstep}{(#3-#2)/#4}
  \bargridlines{#1}{#2}{#3}{\bargridlinesstep}
}

% \barfillrectat{point}{width}{height}{color}{pattern}: draw a
% black-outlined rectangle with corner at `point` (a coordinate, e.g.
% "(0.3,0)" or "(somenode.east)"), filled per `pattern`
% (full/striped/dotted, see the "bar fill ..." styles above), in `color`.
\newcommand{\barfillrectat}[5]{%
  \begingroup
    \edef\barfillpattern{#5}%
    \def\barfillfullname{full}%
    \def\barfillstripedname{striped}%
    \ifx\barfillpattern\barfillfullname
      \filldraw[bar fill full={#4}, draw=black, line width=0.5pt] #1 rectangle ++(#2,#3);
    \else\ifx\barfillpattern\barfillstripedname
      \filldraw[bar fill striped={#4}, draw=black, line width=0.5pt] #1 rectangle ++(#2,#3);
    \else
      \filldraw[bar fill dotted={#4}, draw=black, line width=0.5pt] #1 rectangle ++(#2,#3);
    \fi\fi
  \endgroup
}

% \drawbar{c}{value}{vmin}{vmax}{color}{thickness}{pattern}: draw a single
% bar whose top edge is `c` cm below the top of the diagram, from the
% baseline (x=0) out to `value`, scaled against \barchartlength over the
% [vmin,vmax] range. `pattern` selects the filling setting: full (solid),
% striped, or dotted.
\newcommand{\drawbar}[7]{%
  \pgfmathsetmacro{\drawbarlen}{(#2-#3)/(#4-#3)*\barchartlength}
  \pgfmathsetmacro{\drawbary}{-(#1)}
  \pgfmathsetmacro{\drawbarneg}{-(#6)}
  \barfillrectat{(0,\drawbary)}{\drawbarlen}{\drawbarneg}{#5}{#7}
}

% \barvaluelabel{c}{value}{vmin}{vmax}{thickness}: numeric label just past
% the end of a bar (same `c`/`thickness` as the matching \drawbar).
\newcommand{\barvaluelabel}[5]{%
  \pgfmathsetmacro{\barlabelx}{(#2-#3)/(#4-#3)*\barchartlength+0.05}
  \pgfmathsetmacro{\barlabely}{-(#1+#5/2)}
  \node[bar value label] at (\barlabelx,\barlabely) {#2};
}

% \barcategorylabel{c}{thickness}{text}: category label centered against a
% bar (or group of bars) `c` cm below the top, to the left of the baseline.
\newcommand{\barcategorylabel}[3]{%
  \pgfmathsetmacro{\barlabely}{-(#1+#2/2)}
  \node[bar label, anchor=east] at (-0.15,\barlabely) {#3};
}

% \baraxistitle[offset]{span}{text}: horizontal title of the value axis,
% centered under the tick labels drawn by \bargridlines. `offset` is the
% distance from the value axis to the top of the title (default 0.5 clears
% the tick labels).
\newcommand{\baraxistitle}[3][0.5]{%
  \node[bar label, anchor=north] at (\barchartlength/2,-#2-#1) {#3};
}

% \listlength{list}{\lenmacro}: count the comma-separated entries in `list`
% and store the result (as a plain number) in \lenmacro. E.g.
%   \def\models{Haiku,Sonnet,Opus,Terra}
%   \listlength{\models}{\nmodels} % \nmodels expands to 4
\newcount\listlengthcounter
\newcommand{\listlength}[2]{%
  \global\listlengthcounter=0
  \foreach \listlengthelt in #1 {\global\advance\listlengthcounter by 1}
  \xdef#2{\number\listlengthcounter}
}

% \nthitem{list}{index}{\resultmacro}: store the 0-based `index`-th
% comma-separated entry of `list` into \resultmacro. E.g.
%   \def\dataA{55,68,82,77}
%   \nthitem{\dataA}{2}{\val} % \val expands to 82
% Useful to look up a per-model value while looping over a separate list
% (e.g. \models) that carries the matching names/colors.
\newcommand{\nthitem}[3]{%
  \foreach \nthitemval [count=\nthitemidx from 0] in #1 {%
    \ifnum\nthitemidx=#2
      \protected@xdef#3{\nthitemval}%
    \fi
  }%
}

% Legend geometry. Redefine before \input to override.
\providecommand{\barlegendswatchsize}{0.25} % legend square width/height
\providecommand{\barlegendtextgap}{0}       % square -> its label
\providecommand{\barlegendentrygap}{0.25}   % label -> next entry's square
\providecommand{\barlegendleftmargin}{0}    % row start x
\providecommand{\barlegendgroupgap}{1}      % extra gap between legend groups

% \barlegendreset[x]{y}: start a new legend row at height y, at x
% (default \barlegendleftmargin -- override when the diagrams themselves
% aren't anchored at x=0, e.g. centered layouts using negative xshifts).
% Call once per row, before any \barlegendentry / \barlegendpatternentry
% calls for that row.
\newcommand{\barlegendreset}[2][\barlegendleftmargin]{%
  \xdef\barlegendrowy{#2}
  \coordinate (barlegendcursor) at (#1,#2);
}

% Internal: draw one legend entry (swatch + label) at the current cursor,
% then advance the cursor to just after the label -- so entries "stack"
% tightly, each one starting right where the previous label ended, rather
% than at fixed/hand-tuned x offsets. `text height`/`text depth` are fixed
% so different labels (e.g. "Opus" vs "rocq-mcp") center on their swatch
% identically, regardless of ascenders/descenders/hyphens in the text.
% The row's y always comes from \barlegendrowy (fixed by \barlegendreset),
% never from \barlegendcursor's own y -- \barlegendcursor only tracks x
% (via each label's measured .east anchor); reusing its y directly would
% compound a swatchsize/2 drift onto every following entry.
\newcount\barlegendcounter
\newcommand{\barlegendsharedentry}[3]{%
  \global\advance\barlegendcounter by 1
  \edef\barlegendnodename{barlegendlabel\the\barlegendcounter}
  \barfillrectat{(barlegendcursor |- 0,\barlegendrowy)}{\barlegendswatchsize}{\barlegendswatchsize}{#1}{#2}
  \node[bar label, anchor=west, text height=1.5ex, text depth=.25ex,
        name=\barlegendnodename] at
    ($(barlegendcursor |- 0,\barlegendrowy)+(\barlegendswatchsize+\barlegendtextgap,\barlegendswatchsize/2)$) {#3};
  \coordinate (barlegendcursor) at ($(\barlegendnodename.east)+(\barlegendentrygap,0)$);
}

% \barlegendgroupbreak: insert \barlegendgroupgap of extra horizontal space
% before the next entry, without drawing anything -- use it between two
% "groups" of legend entries on the same row (e.g. models vs. toolings)
% that should be visually separated a bit more than entries within a group.
\newcommand{\barlegendgroupbreak}{%
  \coordinate (barlegendcursor) at ($(barlegendcursor)+(\barlegendgroupgap,0)$);
}

% \barlegendentry{color}{text}: a small solid-colored swatch + label,
% chained after the previous entry on the current row (see \barlegendreset).
\newcommand{\barlegendentry}[2]{\barlegendsharedentry{#1}{full}{#2}}

% \barlegendpatternentry{pattern}{text}: a small neutral-colored swatch
% showing `pattern` (full/striped/dotted) + label, chained the same way --
% for a legend row that identifies patterns (e.g. a tooling/setting)
% independent of color.
\newcommand{\barlegendpatternentry}[2]{\barlegendsharedentry{black!60}{#1}{#2}}

% \barchartmax{list}{\resultmacro}: given a list of brace-grouped value
% sublists (e.g. \dataA below), find the maximum value across all of them
% and store 1.15x that (a bit of headroom) into \resultmacro. Handy to
% auto-scale a diagram's ymax to whatever data it's given. E.g.
%   \def\dataA{{44},{50,73,82}}
%   \barchartmax{\dataA}{\ymaxA} % \ymaxA expands to 94.3
\newcommand{\barchartmax}[2]{%
  \xdef\barchartmaxval{0}
  \foreach \barchartmaxsub in #1 {
    \foreach \barchartmaxelt in \barchartmaxsub {
      \pgfmathparse{max(\barchartmaxval,\barchartmaxelt)}
      \xdef\barchartmaxval{\pgfmathresult}
    }
  }
  \pgfmathsetmacro{#2}{\barchartmaxval*1.15}
}

% \barchartnbars{list}{\resultmacro}: total count of values across all the
% brace-grouped sublists of `list` (see \barchartmax). Useful to size a
% diagram that groups a variable number of bars per category.
\newcommand{\barchartnbars}[2]{%
  \xdef\barchartnbarscount{0}
  \foreach \barchartnbarssub in #1 {
    \foreach \barchartnbarselt in \barchartnbarssub {
      \pgfmathparse{\barchartnbarscount+1}
      \xdef\barchartnbarscount{\pgfmathresult}
    }
  }
  \xdef#2{\barchartnbarscount}
}

% \splitpair{pair}{\namemacro}{\valmacro}: split a "name/value" macro or
% text `pair` into its two halves. Fully expands `pair` first, so it also
% works when `pair` is itself a macro (e.g. from \nthitem) rather than
% literal text -- plain "\foreach \a/\b in {\pairmacro}" does NOT reliably
% split in that case, since foreach doesn't force-expand a lone macro token
% sitting inside an inline {...} list to find the "/".
\newcommand{\splitpair}[3]{%
  \protected@edef\splitpairtmp{#1}%
  \foreach \splitpaira/\splitpairb in \splitpairtmp {
    \protected@xdef#2{\splitpaira}%
    \protected@xdef#3{\splitpairb}%
  }
}

% \plotseries{points}{xmax}{vmin}{vmax}{width}{height}{color}: draw a
% connected line with filled circle markers through `points` (an
% "idx/value" list, e.g. {0/33,1/38,5/48}), mapping idx in [0,xmax]
% linearly to x in [0,width] and value in [vmin,vmax] to y in [0,height].
% For a chart with a category axis (idx) and a value axis (value), e.g.
% accuracy against a chronological feature index.
%   \pgfmathsetmacro is NOT safe to call from inside a \foreach that is
%   itself feeding a \draw path (TikZ's path parser wants only path syntax
%   there, not arbitrary macro calls -- it fails with "Giving up on this
%   path"): so this first collects every point into a plain coordinate-list
%   macro in an ordinary \foreach, then draws that list in one separate
%   \draw ... plot coordinates {...}.
% Stroke width of the connecting line. Redefine before \input to override,
% e.g. \renewcommand{\plotserieslinewidth}{1.5pt}.
\providecommand{\plotserieslinewidth}{1.5pt}
% \plotseriesline / \plotseriesdots draw the two halves of \plotseries
% separately (same arguments), for a series whose markers aren't all the
% same -- e.g. a line whose last point is a \plotcrosses cross instead.
\newcommand{\plotseriesline}[7]{%
  \xdef\plotseriescoords{}
  \foreach \plotseriesidx/\plotseriesval in #1 {
    \pgfmathsetmacro{\plotseriesx}{\plotseriesidx/#2*#5}
    \pgfmathsetmacro{\plotseriesy}{(\plotseriesval-#3)/(#4-#3)*#6}
    \ifx\plotseriescoords\empty
      \xdef\plotseriescoords{(\plotseriesx,\plotseriesy)}
    \else
      \xdef\plotseriescoords{\plotseriescoords (\plotseriesx,\plotseriesy)}
    \fi
  }
  \draw[#7, line width=\plotserieslinewidth] plot coordinates {\plotseriescoords};
}
\newcommand{\plotseriesdots}[7]{%
  \foreach \plotseriesidx/\plotseriesval in #1 {
    \pgfmathsetmacro{\plotseriesx}{\plotseriesidx/#2*#5}
    \pgfmathsetmacro{\plotseriesy}{(\plotseriesval-#3)/(#4-#3)*#6}
    \filldraw[fill=#7, draw=none] (\plotseriesx,\plotseriesy) circle (2.5pt);
  }
}
\newcommand{\plotseries}[7]{%
  \plotseriesline{#1}{#2}{#3}{#4}{#5}{#6}{#7}
  \plotseriesdots{#1}{#2}{#3}{#4}{#5}{#6}{#7}
}

% \plotcrosses{points}{xmax}{vmin}{vmax}{width}{height}{color}: like
% \plotseriesdots, but a cross (x) at each point instead of a filled dot,
% and no connecting line -- e.g. to mark data points of rejected
% mutations. Size/stroke: \plotcrosssize (half-extent) and
% \plotcrosslinewidth, redefinable like \plotserieslinewidth above.
\providecommand{\plotcrosssize}{3pt}
\providecommand{\plotcrosslinewidth}{1.2pt}
\newcommand{\plotcrosses}[7]{%
  \foreach \plotseriesidx/\plotseriesval in #1 {
    \pgfmathsetmacro{\plotseriesx}{\plotseriesidx/#2*#5}
    \pgfmathsetmacro{\plotseriesy}{(\plotseriesval-#3)/(#4-#3)*#6}
    \begin{scope}[shift={(\plotseriesx,\plotseriesy)}]
      \draw[#7, line width=\plotcrosslinewidth]
        (-\plotcrosssize,-\plotcrosssize) -- (\plotcrosssize,\plotcrosssize)
        (-\plotcrosssize,\plotcrosssize) -- (\plotcrosssize,-\plotcrosssize);
    \end{scope}
  }
}

% \plotcrosslinks{base}{crosses}{xmax}{vmin}{vmax}{width}{height}{color}:
% a dotted line from the point `base` (one "idx/value" pair, as a macro,
% e.g. the last accepted point) to each point of `crosses` (an "idx/value"
% list, as a macro) -- linking rejected data points back to the valid one
% they were compared against. Draw it BEFORE the series/crosses so their
% markers sit on top. The dot pattern is the `bar link` style below.
\tikzset{bar link/.style={line cap=round, dash pattern=on 0pt off 3.5pt}}
\newcommand{\plotcrosslinks}[8]{%
  \foreach \plotlinkbidx/\plotlinkbval in #1 {
    \pgfmathsetmacro{\plotlinkbx}{\plotlinkbidx/#3*#6}
    \pgfmathsetmacro{\plotlinkby}{(\plotlinkbval-#4)/(#5-#4)*#7}
    \foreach \plotlinkcidx/\plotlinkcval in #2 {
      \pgfmathsetmacro{\plotlinkcx}{\plotlinkcidx/#3*#6}
      \pgfmathsetmacro{\plotlinkcy}{(\plotlinkcval-#4)/(#5-#4)*#7}
      \draw[#8, line width=\plotserieslinewidth, bar link]
        (\plotlinkbx,\plotlinkby) -- (\plotlinkcx,\plotlinkcy);
    }
  }
}

% \plotbands{idxlist}{xmax}{width}{height}: a light gray background band
% behind each idx in `idxlist` (a comma list, passed as a macro like the
% other list arguments), one category slot wide (width/xmax) and centered
% on the idx, spanning [0,height] vertically -- to flag categories that
% are special, e.g. rejected mutations. Draw it BEFORE gridlines/series so
% it sits behind them; adjacent idxs merge into a single block.
\tikzset{bar reverted band/.style={fill=gray!22, draw=none}}
\newcommand{\plotbands}[4]{%
  \foreach \plotbandidx in #1 {
    \pgfmathsetmacro{\plotbandleft}{(\plotbandidx-0.5)/#2*#3}
    \pgfmathsetmacro{\plotbandright}{(\plotbandidx+0.5)/#2*#3}
    \path[bar reverted band] (\plotbandleft,0) rectangle (\plotbandright,#4);
  }
}

% \plotbugbands{idxlist}{xmax}{width}{height}: like \plotbands, but a gray
% diagonal-hatched band instead of a solid one -- to flag categories that are
% special without being rejected, e.g. a bug-fix mutation (kept, but not a
% feature).
\tikzset{bar bugfix band/.style={pattern={Lines[angle=45, distance=3pt, line width=0.4pt]}, pattern color=gray!60, draw=none}}
\newcommand{\plotbugbands}[4]{%
  \foreach \plotbandidx in #1 {
    \pgfmathsetmacro{\plotbandleft}{(\plotbandidx-0.5)/#2*#3}
    \pgfmathsetmacro{\plotbandright}{(\plotbandidx+0.5)/#2*#3}
    \path[bar bugfix band] (\plotbandleft,0) rectangle (\plotbandright,#4);
  }
}

% \vxticksNum[offset]{xmax}{width}: a category-axis baseline with a tick and a
% plain centered number (offset..offset+xmax; offset defaults to 0) under it at each of the xmax+1 slots
% spanning [0,width] -- for when the category names are given elsewhere
% (a key) and only their indices label the axis. See \vxticks for named,
% rotated labels instead.
\newcommand{\vxticksNum}[3][0]{%
  \draw[bar axis] (0,0) -- (#3,0);
  \foreach \vxnumi in {0,...,#2} {
    \pgfmathsetmacro{\vxnumpos}{\vxnumi/#2*#3}
    \pgfmathtruncatemacro{\vxnumlabel}{\vxnumi+#1}
    \draw[bar axis] (\vxnumpos,0) -- (\vxnumpos,-0.08);
    \node[bar tick label, anchor=north] at (\vxnumpos,-0.1) {\vxnumlabel};
  }
}

% \vaxisgridlines{width}{height}{vmin}{vmax}{ystep}{precision}: for a
% \plotseries-style chart (vertical value axis, horizontal category axis).
% Draw horizontal gray gridlines every `ystep` data units from vmin to
% vmax, mapped onto [0,height], with left-side numeric tick labels rounded
% to `precision` decimals, plus the left (value) axis line. No bottom
% (category baseline) line is drawn -- for a chart whose category axis is
% shared across several stacked/juxtaposed diagrams, draw that once
% separately (see \vxticksTop for a version floating above the diagrams,
% labels pointing up) rather than once per diagram here. `ystep` should
% evenly divide (vmax-vmin); \vaxisgridlinesN below picks it automatically
% for a given number of equal gridline gaps instead.
\newcommand{\vaxisgridlines}[6]{%
  % floor(...+epsilon): (vmax-vmin)/ystep is meant to be an exact integer,
  % but floating point can land it a hair under (e.g. 2.99988 instead of
  % 3), silently dropping the last gridline from the {0,...,n} loop below.
  \pgfmathsetmacro{\vaxisnsteps}{floor((#4-#3)/#5+0.001)}
  \foreach \i in {0,...,\vaxisnsteps} {
    \pgfmathsetmacro{\vaxisval}{#3+\i*#5}
    \pgfmathsetmacro{\vaxispos}{(\vaxisval-#3)/(#4-#3)*#2}
    \draw[bar grid] (0,\vaxispos) -- (#1,\vaxispos);
    \node[bar tick label, anchor=east] at (-0.15,\vaxispos) {\pgfmathprintnumber[fixed,precision=#6,zerofill=false]{\vaxisval}};
  }
  \draw[bar axis] (0,0) -- (0,#2);
}

% \vaxisgridlinesRight{width}{height}{vmin}{vmax}{ystep}{precision}: like
% \vaxisgridlines, but with the tick labels and the axis line on the RIGHT
% edge (x=width) -- for a second value scale, e.g. a later phase measured
% on another scale, drawn next to the first one. Keep the same number of
% steps (vmax-vmin)/ystep as the left-hand axis of the same panel so the
% two share their gridline heights.
\newcommand{\vaxisgridlinesRight}[6]{%
  \pgfmathsetmacro{\vaxisnsteps}{floor((#4-#3)/#5+0.001)}
  \foreach \i in {0,...,\vaxisnsteps} {
    \pgfmathsetmacro{\vaxisval}{#3+\i*#5}
    \pgfmathsetmacro{\vaxispos}{(\vaxisval-#3)/(#4-#3)*#2}
    \draw[bar grid] (0,\vaxispos) -- (#1,\vaxispos);
    \node[bar tick label, anchor=west] at (#1+0.15,\vaxispos) {\pgfmathprintnumber[fixed,precision=#6,zerofill=false]{\vaxisval}};
  }
  \draw[bar axis] (#1,0) -- (#1,#2);
}

% \vseparator{height}: a vertical bar of the given height at the current
% origin, to separate regions of a diagram (e.g. two phases).
\tikzset{bar separator/.style={draw=black!70, line width=1pt}}
\newcommand{\vseparator}[1]{\draw[bar separator] (0,0) -- (0,#1);}

% \vaxisgridlinesN{width}{height}{vmin}{vmax}{n}{precision}: like
% \vaxisgridlines, but takes a number of equal gridline gaps `n` instead of
% an explicit ystep.
\newcommand{\vaxisgridlinesN}[6]{%
  \pgfmathsetmacro{\vaxisstepN}{(#4-#3)/#5}
  \vaxisgridlines{#1}{#2}{#3}{#4}{\vaxisstepN}{#6}
}

% \vaxistitle[xoffset]{height}{text}: rotated title of the value axis drawn
% by \vaxisgridlines, vertically centered against it. Default xoffset=-0.9
% clears two-digit tick labels; make it more negative for wider ticks.
\newcommand{\vaxistitle}[3][-0.9]{%
  \node[bar label, rotate=90, anchor=south] at (#1,#2/2) {#3};
}

% \vxticks{list}{xmax}{width}: a category-axis baseline with ticks and
% rotated labels below it, for a "idx/name" `list` (e.g. the same list
% \plotseries's `points` are indexed against), idx in [0,xmax] mapped to x
% in [0,width]. Meant to be drawn once, e.g. floating below a stack of
% diagrams sharing this category axis (see \vaxisgridlines, which does not
% draw its own per-diagram baseline); \vxticksTop is the mirror image, for
% floating above instead, labels pointing up.
\newcommand{\vxticks}[3]{%
  \draw[bar axis] (0,0) -- (#3,0);
  \foreach \vxtickidx/\vxtickname in #1 {
    \pgfmathsetmacro{\vxtickpos}{\vxtickidx/#2*#3}
    \draw[bar axis] (\vxtickpos,0) -- (\vxtickpos,-0.08);
    \node[bar tick label, rotate=60, anchor=east, font=\scriptsize] at (\vxtickpos,-0.12) {\vxtickname};
  }
}

% \vxticksTop{list}{xmax}{width}: like \vxticks, but floating above the
% diagram(s) instead of below -- a horizontal baseline with tick marks
% pointing up and rotated labels reading upward. Meant to be drawn once,
% at the top of a stack of diagrams sharing this category axis (see
% \vaxisgridlines, which no longer draws its own per-diagram baseline).
\newcommand{\vxticksTop}[3]{%
  \draw[bar axis] (0,0) -- (#3,0);
  \foreach \vxtickidx/\vxtickname in #1 {
    \pgfmathsetmacro{\vxtickpos}{\vxtickidx/#2*#3}
    \draw[bar axis] (\vxtickpos,0) -- (\vxtickpos,0.08);
    \node[bar tick label, rotate=60, anchor=west, font=\scriptsize] at (\vxtickpos,0.12) {\vxtickname};
  }
}

% \bargroupedbars{modelslist}{data}{toolingslist}{vmin}{vmax}{thickness}{groupgap}:
% draw one group of bars per model in `modelslist` (a "Name/color" list,
% e.g. \models), at the current origin, the first model at the top. `data`
% holds one brace-grouped value sublist per model, in the same order as
% `modelslist` (see \barchartmax for the shape). `data`'s per-model sublist
% may be SHORTER than `toolingslist` (a "Name/pattern" list, e.g.
% \toolings): if so, its values are matched to the LAST entries of
% `toolingslist` (so a single-value sublist means "only tried with the last
% tooling"). Bars are `thickness` cm thick, touching within a group, with
% `groupgap` cm between groups (and before the first / after the last);
% each is colored by its model and patterned by its tooling.
\newcommand{\bargroupedbars}[7]{%
  \listlength{#3}{\bargroupedntoolings}
  \xdef\bargroupedcursor{#7}
  \foreach \bargroupedmodel/\bargroupedcol [count=\bargroupedi from 0] in #1 {
    \nthitem{#2}{\bargroupedi}{\bargroupedmodeldata}
    \listlength{\bargroupedmodeldata}{\bargroupedsublen}
    \pgfmathtruncatemacro{\bargroupedoffset}{\bargroupedntoolings-\bargroupedsublen}
    \foreach \bargroupedval [count=\bargroupedj from 0] in \bargroupedmodeldata {
      \pgfmathtruncatemacro{\bargroupedtidx}{\bargroupedoffset+\bargroupedj}
      \nthitem{#3}{\bargroupedtidx}{\bargroupedtoolpair}
      \splitpair{\bargroupedtoolpair}{\bargroupedtoolname}{\bargroupedpattern}
      \drawbar{\bargroupedcursor}{\bargroupedval}{#4}{#5}{\bargroupedcol}{#6}{\bargroupedpattern}
      % \barvaluelabel{\bargroupedcursor}{\bargroupedval}{#4}{#5}{#6}
      \pgfmathparse{\bargroupedcursor+#6}
      \xdef\bargroupedcursor{\pgfmathresult}
    }
    \pgfmathparse{\bargroupedcursor+#7}
    \xdef\bargroupedcursor{\pgfmathresult}
  }
}

% ---------------------------------------------------------------------------
% Example usage (single-series bar chart) — copy into a figure and adapt:
%
% \input{figures/barchart-defs.tex}
% \begin{tikzpicture}
%   \def\vmin{0}
%   \def\vmax{100}
%   \def\span{1.6}                         % extent along the category direction
%   \bargridlinesN{\span}{\vmin}{\vmax}{5} % 5 equal gridline gaps
%   \baraxes{\span}
%   \baraxistitle{\span}{Accuracy (\%)}
%   \drawbar{0.3}{72}{\vmin}{\vmax}{barcolorA}{0.5}{full}
%   \barvaluelabel{0.3}{72}{\vmin}{\vmax}{0.5}
%   \barcategorylabel{0.3}{0.5}{Baseline}
%   \drawbar{0.9}{88}{\vmin}{\vmax}{barcolorB}{0.5}{striped}
%   \barvaluelabel{0.9}{88}{\vmin}{\vmax}{0.5}
%   \barcategorylabel{0.9}{0.5}{Ours}
% \end{tikzpicture}
%
% For grouped bars, call \drawbar/\barvaluelabel repeatedly at c, c+thickness,
% etc. within a group, then leave a gap before the next group's c.
% The `pattern` argument of \drawbar (full/striped/dotted) is independent of
% `color` -- e.g. use it to distinguish a setting (one pattern per diagram)
% while color still distinguishes each bar/model within that diagram.
% ---------------------------------------------------------------------------
\makeatother

